Highly Efficient Test-Time Scaling for T2I Diffusion Models with Text Embedding Perturbation

Test-time scaling (TTS) aims to achieve better results by increasing random sampling and evaluating samples based on rules and metrics. However, in text-to-image(T2I) diffusion models, most related works focus on search strategies and reward models, yet the impact of the stochastic characteristic of noise in T2I diffusion models on the method's performance remains unexplored. In this work, we analyze the effects of randomness in T2I diffusion models and explore a new format of randomness for TTS: text embedding perturbation, which couples with existing randomness like SDE-injected noise to enhance generative diversity and quality. We start with a frequency-domain analysis of these formats of randomness and their impact on generation, and find that these two randomness exhibit complementary behavior in the frequency domain: spatial noise favors low-frequency components (early steps), while text embedding perturbation enhances high-frequency details (later steps), thereby compensating for the potential limitations of spatial noise randomness in high-frequency manipulation. Concurrently, text embedding demonstrates varying levels of tolerance to perturbation across different dimensions of the generation process. Specifically, our method consists of two key designs: (1) Introducing step-based text embedding perturbation, combining frequency-guided noise schedules with spatial noise perturbation. (2) Adapting the perturbation intensity selectively based on their frequency-specific contributions to generation and tolerance to perturbation. Our approach can be seamlessly integrated into existing TTS methods and demonstrates significant improvements on multiple benchmarks with almost no additional computation. Code is available at \href{https://github.com/xuhang07/TEP-Diffusion}{https://github.com/xuhang07/TEP-Diffusion}.

==> tab/sd2_1.tex <==
\begin{table*}[t]
\centering
\begin{small}



\begin{tabular}{ccccccc}
\toprule
Sampling Method &w/ TEP & HPSv2$\uparrow$ & ImageReward$\uparrow$ & CLIPScore$\uparrow$ &AestheticScore$\uparrow$ &GenEval$\uparrow$\\ \hline\hline
None(SD2.1) & \ding{55} &0.264 &-0.020 &18.30 &5.287 &0.48\\ \hline\hline
\multicolumn{7}{c}{ODE-Based Methods} \\ \hline\hline
\multirow{2}{*}{BoN~\cite{ma2025inference}} &\ding{55} &0.278 &0.910 &18.42 &5.985 &0.54 \\
&\ding{51} &\textbf{0.286} &\textbf{0.956} &\textbf{19.19} &\textbf{6.124} &\textbf{0.55}\\ \hline
\multirow{2}{*}{ZeroOrder~\cite{ma2025inference}} &\ding{55} &0.281 &0.856 &19.23 &5.999 &0.57\\
&\ding{51} &\textbf{0.286} &\textbf{0.912} &\textbf{19.39} &\textbf{6.043} &\textbf{0.62}\\ \hline\hline
\multicolumn{7}{c}{Particle Sampling Methods} \\ \hline\hline
\multirow{2}{*}{CoDe~\cite{singh2025code}} &\ding{55} &0.279 &0.945 &19.23 &6.036 &0.61\\
&\ding{51} &\textbf{0.291} &\textbf{1.158} &\textbf{19.59} &\textbf{6.338} &\textbf{0.73}\\ \hline
\multirow{2}{*}{SVDD~\cite{li2024derivative}} &\ding{55} &0.283 &1.265 &19.75 &6.323 &0.61\\
&\ding{51} &\textbf{0.294} &\textbf{1.380} &\textbf{19.94} &\textbf{6.573} &\textbf{0.67}\\ \hline
\multirow{2}{*}{DAS~\cite{kim2025test}} &\ding{55} &0.277 &0.922 &19.17 &5.998 &0.58\\
&\ding{51} &\textbf{0.287} &\textbf{1.028} &\textbf{19.18} &\textbf{6.238} &\textbf{0.63}\\ \hline\hline
\multicolumn{7}{c}{Resampling-Based Methods} \\ \hline\hline
\multirow{2}{*}{SoP~\cite{ma2025inference}} &\ding{55} &0.282 &0.934 &18.49 &6.021 &0.60\\
&\ding{51} &\textbf{0.288} &\textbf{0.971} &\textbf{19.10} &\textbf{6.281} &\textbf{0.64}\\ \hline

\bottomrule
\end{tabular}
\caption{Results of test-time scaling methods w/ and w/o our framework on SD v2.1.}
\label{tab:sd2}
\end{small}
\end{table*}
